The Configurable SAT Solver Challenge (CSSC)

It is well known that different solution strategies work well for different types of instances of hard combinatorial problems. As a consequence, most solvers for the propositional satisfiability problem (SAT) expose parameters that allow them to be customized to a particular family of instances. In the international SAT competition series, these parameters are ignored: solvers are run using a single default parameter setting (supplied by the authors) for all benchmark instances in a given track. While this competition format rewards solvers with robust default settings, it does not reflect the situation faced by a practitioner who only cares about performance on one particular application and can invest some time into tuning solver parameters for this application. The new Configurable SAT Solver Competition (CSSC) compares solvers in this latter setting, scoring each solver by the performance it achieved after a fully automated configuration step. This article describes the CSSC in more detail, and reports the results obtained in its two instantiations so far, CSSC 2013 and 2014.

==> benchmark_table.tex <==
%\begin{table}
%\sffamily\small\centering%
%\begin{tabular}{@{}l l l l r}
%\toprule[1.0pt]
%
%Benchmark & \# Variables & \# Clauses & Years used & Reference\\
%\midrule
%
%\swvshort & $68\,935 \pm 56\,966$ & $181\,714 \pm 206\,147$ & 2013 & \cite{babic-hvc07}\\
%\myrowcolour{}\hwshort & $96\,454 \pm 169\,859$ & $413\,143 \pm 717\,379$ & 2013 \& 2014 & \cite{zarpas-sat05a}\\
%\circuit &$5\,532 \pm 7\,453$ & $18\,800 \pm 25\,351$ & 2013 \& 2014 & \cite{brummayer-sat10a}\\
%\myrowcolour{}\bmcshort{} & $424\,136 \pm 842\,859$ & $1\,029\,240 \pm 2\,297\,554$ & 2013 \& 2014 & \cite{biere-misc08a}\\
%
%\midrule
%
%\gishort & $11\,170 \pm 17\,796$ & $2\,982\,037 \pm 8\,027\,141$ & 2013 \& 2014 & ?\\
%\myrowcolour{}\labsshort & $75\,926 \pm 75\,668$ & $154\,032 \pm 153\,043$ & 2013 \& 2014 & ?\\
%\queens & $38\,193 \pm 37\,415$ & $124\,948 \pm 126\,280$ & 2014 & \\
%
%\midrule
%
%\myrowcolour{}\kthree & $262 \pm 43$ & $1116 \pm 182$ & 2013 \& 2014 & ?\\
%\threecnf{} & $350 \pm 0$ & $1493 \pm 0$ & 2014 & ?\\
%\myrowcolour{}\unif & $50 \pm 0$ & $1056 \pm 0$ & 2013 \& 2014 & ?\\
%
%\midrule
%
%\threesatonek & $500 \pm 0$ & $10000 \pm 0$ & 2013 \& 2014 & ?\\
%\myrowcolour{}\fivesatfiveh & $1000 \pm 0$ & $4260 \pm 0$ & 2014 & ?\\
%\sevensatninety & $90 \pm 0$ & $7650 \pm 0$ & 2014 & ?\\
%
%\bottomrule[1.0pt]
%
%\end{tabular}
%\caption{Overview of benchmark sets used.\label{tab:benchmarks}}
%
%\end{table}



\begin{table}
\sffamily\small\centering%
\begin{tabular}{@{}l l l l l l r}
\toprule[1.0pt]

Benchmark & \#Train/Test & \#Variables & \#Clauses & Years used & Ref.\\
\midrule
%\cmidrule[0.6pt](r{0.25em}){1-1}% horizontal line, 1.0pt think, from column 1 to column 1, trim 0.25em on right side.
%\cmidrule[0.6pt](lr{0.125em}){2-2}% horizontal line, 1.0pt think, from column 2 to column 2, trim 0.125em on each of left and right side.
%\cmidrule[0.6pt](lr{0.125em}){3-3}%
%\cmidrule[0.6pt](lr{0.125em}){4-4}%
%\cmidrule[0.6pt](lr{0.125em}){5-5}%
%\cmidrule[1.0pt](lr{0.125em}){10-11}%
%\cmidrule[1.0pt](l{0.25em}){12-13}%
% \midrule

\swvshort & 302/302 & $68.9k \pm 57.0k$ & $182k \pm 206k$ & 2013 & \cite{babic-hvc07}\\
\myrowcolour{}\hwshort & 382/383 & $96.4k \pm 170k$ & $413k \pm 717k$ & 2013 \& 2014 & \cite{zarpas-sat05a}\\
\circuit & 299/585 &$5.53k \pm 7.45k$ & $18.8k \pm 25.3k$ & 2013 \& 2014 & \cite{brummayer-sat10a}\\
\myrowcolour{}\bmcshort{} & 807/807 & $424k \pm 843k$ & $1.03m \pm 2.30m$ & 2013 \& 2014 & \cite{biere-misc08a}\\

\midrule

\gishort & 1032/1032 & $11.2k \pm 17.8k$ & $2.98m \pm 8.03m$ & 2013 \& 2014 & ?\\
\myrowcolour{}\labsshort & 350/351 & $75.9k \pm 75.7k$ & $154k \pm 153k$ & 2013 \& 2014 & ?\\
\queens & 484/351 & $38.2k \pm 37.4k$ & $125k \pm 126k$ & 2014 & \cite{manthey-sat14r}\\

\midrule

\myrowcolour{}\kthree & 300/300 & $262 \pm 43$ & $1116 \pm 182$ & 2013 \& 2014 & \cite{bayless-lion14a}\\
\threecnf{} & 500/250 & $350 \pm 0$ & $1493 \pm 0$ & 2014 & \cite{bebel-sat13a}\\
\myrowcolour{}\unif & 300/300 & $50 \pm 0$ & $1056 \pm 0$ & 2013 \& 2014 & ?\\

\midrule

\threesatonek & 250/250 & $500 \pm 0$ & $10000 \pm 0$ & 2013 \& 2014 & \cite{tompkins-sat11}\\
\myrowcolour{}\fivesatfiveh & 250/250 & $1000 \pm 0$ & $4260 \pm 0$ & 2014 & \cite{tompkins-sat11}\\
\sevensatninety & 250/250 & $90 \pm 0$ & $7650 \pm 0$ & 2014 & \cite{tompkins-sat11}\\

\bottomrule[1.0pt]

\end{tabular}
\caption{Overview of benchmark sets used.\label{tab:benchmarks-v2}}

\end{table}


==> scenario_results_table.tex <==
\begin{table}[tp]
\sffamily\small\centering
\begin{tabular}{l | ccc}
\toprule[1.0pt]
& \multicolumn{3}{c}{\indu}\\
 & \bmc & \circuit & \hw \\
\midrule
\riss & $421.47 \to \mathbf{285.07}$ & $218.11 \to 233.90$ & $721.03 \to \mathbf{720.54}$\\
\myrowcolour{}\sparrow & $744.44 \to \mathbf{382.71}$ & $433.06 \to \mathbf{227.41}$ & $798.05 \to \mathbf{723.74}$\\
\clasp & $451.13 \to \mathbf{315.50}$ & $193.53 \to \mathbf{134.91}$ & $710.36 \to 710.01$\\
\myrowcolour{}\cryptominisat & $428.49 \to 405.26$ & $328.41 \to \mathbf{214.90}$ & $703.30 \to 695.47$\\
\lingeling & $222.46 \to \mathbf{221.37}$ & $316.00 \to \mathbf{192.88}$ & $697.30 \to \mathbf{694.08}$\\
\myrowcolour{}\minisathack & $233.16 \to 231.56$ & $226.20 \to 204.16$ & $698.74 \to \mathbf{697.98}$\\
\bottomrule[1.0pt]
& \multicolumn{3}{c}{\crafted}\\
& \gi & \textit{LABS} & \queens \\
\midrule
\riss & $372.32 \to \mathbf{267.32}$ & $789.03 \to 762.65$ & $29.07 \to \mathbf{7.31}$\\
\myrowcolour{}\sparrow & $538.10 \to \mathbf{371.08}$ & $886.06 \to \mathbf{814.01}$ & $115.01 \to \mathbf{8.52}$\\
\yalsat & $1590.73 \to \mathbf{1590.21}$ & $1868.36 \to \mathbf{1776.05}$ & $3000.00 \to 3000.00$\\
\myrowcolour{}\clasp & $370.50 \to \mathbf{89.54}$ & $\mathbf{754.53} \to 803.89$ & $704.92 \to \mathbf{4.68}$\\
\cryptominisat & $369.60 \to \mathbf{219.41}$ & $820.81 \to 774.43$ & $37.94 \to \mathbf{17.32}$\\
\myrowcolour{}\lingeling & $112.10 \to \mathbf{58.28}$ & $873.86 \to 899.05$ & $50.00 \to \mathbf{17.38}$\\
\minisathack & $429.69 \to \mathbf{429.09}$ & $785.44 \to 784.90$ & $11.49 \to \mathbf{8.38}$\\
\bottomrule[1.0pt]
& \multicolumn{3}{c}{\random}\\
& \threecnf & \kthree & \unif \\
\midrule
\dccsat & $91.33 \to \mathbf{18.94}$ & $74.75 \to \mathbf{15.01}$ & $161.57 \to \mathbf{29.90}$\\
\myrowcolour{}\riss & $1969.02 \to \mathbf{1431.21}$ & $49.55 \to 42.06$ & $14.56 \to \mathbf{1.31}$\\
\sparrow & $1517.44 \to 1580.29$ & $176.07 \to \mathbf{31.79}$ & $149.46 \to \mathbf{1.45}$\\
\myrowcolour{}\clasp & $309.48 \to \mathbf{35.03}$ & $7.91 \to \mathbf{2.66}$ & $0.74 \to \mathbf{0.30}$\\
\minisathack & $2039.50 \to \mathbf{1259.23}$ & $84.77 \to \mathbf{25.66}$ & $1.83 \to \mathbf{0.81}$\\
\bottomrule[1.0pt]
& \multicolumn{3}{c}{\randomsat}\\
 & \threesatonek & \fivesatfiveh & \sevensatninety \\
\midrule
\csccsat & $27.24 \to 27.61$ & $\mathbf{6.77} \to 6.80$ & $\mathbf{50.09} \to 84.91$\\
\myrowcolour{}\sparrow & $115.81 \to \mathbf{63.62}$ & $3000.00 \to \mathbf{6.23}$ & $52.15 \to 43.44$\\
\yalsat & $78.07 \to 89.82$ & $4.89 \to 4.60$ & $78.49 \to 75.70$\\
\myrowcolour{}\clasp & $3000.00 \to 3000.00$ & $3000.00 \to 3000.00$ & $3000.00 \to 3000.00$\\
\minisathack & $3000.00 \to 3000.00$ & $3000.00 \to 3000.00$ & $3000.00 \to 3000.00$\\
\myrowcolour{}\probsat & $132.22 \to \mathbf{52.53}$ & $3000.00 \to \mathbf{1.97}$ & $337.30 \to \mathbf{14.72}$\\
\bottomrule[1.0pt]
\end{tabular}
\caption{PAR$10$ performance of default and configured solvers on each scenario of \random. 
The best PAR$10$ values are shown in bold faces where the performance difference 
is statistically significant 
(according to a permutation test with $100\,000$ permutations)
at $\alpha=0.05$.
}
\end{table}



